Effective and General Distance Computation for Approximate Nearest Neighbor Search

Approximate K Nearest Neighbor (AKNN) search in high-dimensional spaces is a critical yet challenging problem. In AKNN search, distance computation is the core task that dominates the runtime. Existing approaches typically use approximate distances to improve computational efficiency, often at the cost of reduced search accuracy. To address this issue, the state-of-the-art method, ADSampling, employs random projections to estimate approximate distances and introduces an additional distance correction process to mitigate accuracy loss. However, ADSampling has limitations in both effectiveness and generality, primarily due to its reliance on random projections for distance approximation and correction. To address the effectiveness limitations of ADSampling, we leverage data distribution to improve distance computation via orthogonal projection. Furthermore, to overcome the generality limitations of ADSampling, we adopt a data-driven approach to distance correction, decoupling the correction process from the distance approximation process. Extensive experiments demonstrate the superiority and effectiveness of our method. In particular, compared to ADSampling, our method achieves a speedup of 1.6 to 2.1 times on real-world datasets while providing higher accuracy.

==> extend.tex <==
\section{Extend Fast Inference}
\subsection{Multiple Linear Models}

We utilize multiple linear models, denoted as $L_1,..,L_n$, each corresponding to a unique projection dimension, with an associated error probability $e_1,..,e_n$ on Label 0 classification. Drawing inspiration from hypothesis testing, if the approximate distance for the current projection dimension is classified as Label 0 by the current linear model $L_i$, we continue to increase the projection dimension. Subsequently, we update the approximate distance and employ the corresponding linear model to make further determinations. This process continues until the project dimension equals the original dimension, at which point we obtain an accurate distance. If this distance is less than the threshold $\tau$, we update the result queue. Then we consider the $r$ recall constraint with multiple linear models.

To achieve the target recall $r$ for Label 0, we need to consider the number of false positives (FP) for each linear model. A straightforward strategy is to set the recall target for each of the $n$ linear models as $r_i= (1 - (1-r)/n)$. This approach ensures that the overall recall target still satisfies the recall constraint for label 0.



\subsection{Extend Model with Quantization}

In addition to random projection and PCA for approximate distance calculations, another popular approach for approximate distance computation is the use of vector quantization methods, with Product Quantization (PQ) being a prominent example. We utilize the distance to quantized centroids of the query $q$ to the database vector $u$ known as the Approximate Distance Computation (ADC), as the approximate distance. We then apply the linear model method with this distance as a feature. The advantage of PQ over projection methods lies in the precomputation of distances between the query point and all quantized centroids, which are stored in a distance look-up table. During distance calculations, only table look-ups are needed, avoiding subtraction and multiplication operations in Euclidean space (which would require three clock cycles and an additional cycle for addition). This optimization leads to a reduction in clock cycles required for distance computation. As the study for the error(distortion) distribution, we can still try to minimize the distortion of PQ. 

Following the same idea as PCA, we use OPQ as our final quantized approximate distance method which also uses an orthogonal matrix to rotate the space. More accurate quantification methods such as AQ\cite{AQ-2014-cvpr}, CompQ\cite{CompQ-2014-ICML}, LSQ\cite{LSQ++-2018-eccv}, and other additional quantization methods are no longer within the scope of our consideration due to their low look-up table efficiency. Furthermore, it is worth considering the incorporation of additional features to achieve even smaller reconstruction errors. For quantization methods, beyond using the distance from query $q$ to the quantized centroid of $q$ as a feature (approximate distance), we can also utilize the distance from $u$ itself to the quantized centroid as an additional feature. This multi-feature approach can further enhance the accuracy of the distance approximation. Moreover, we noticed that PQ has different optimizations with different hardware environments. In our experiments, we additionally analyzed the inference efficiency of using the PQ-scan\cite{PQ-fast-scan-VLDB-2015} as an approximate distance with the SIMD-SSE instruction. As for the In-Register look-up table method\cite{Quicker-adc-PAMI-2019,bolt-KDD-2017}, since it greatly quantizes the distance. For example, mapping the float distance to (0,127) uniformly to make the distance table can be loaded in SSE or AVX Register. This operation will cause great reconstruction loss, which is not considered in this approach.



==> learn-to-prune.tex <==
\section{Learned Fast Inference}

\subsection{Binary Classification With Distance Feature}

To address the above issue, we model the problem of \textit{using approximate distance $dis^{\prime}$ to determine whether the real distance $dis$ exceeds the threshold $\tau$} as a binary-classification problem, in which the label of the two classes is Label 0: $dis \leq \tau$ and Label 1: $dis > \tau$. If we set $\tau$ as the distance from the $k$-th nearest neighbor to the query, then Label 0 will be all the K nearest neighbors of the query, and Label 1 will be the rest. To avoid the calculation of the exact distance, we use the \textbf{approximate distance} $dis^{\prime}$ as the \textbf{feature}, and then a simple linear model $L$ can be used to fast infer whether $dis$ is greater than $\tau$. 
\begin{equation*}
\begin{aligned}
    L(\mathbf{x}) & = sign(w^T\mathbf{x} + b) \\
                  & = \mathbb{I}(m_{1}dis^{\prime} + \beta > \tau)
\end{aligned}
\end{equation*}
Once we have modeled the problem as a linear binary classification problem, the ADsampling method can also be viewed as a linear classifier using approximate distances. The hypothesis test can be rewritten as $L(\textbf{x}) = \mathbb{I}(m \cdot dis^\prime > \tau)$ where $m = 1 / (1+ \epsilon_0\sqrt{d})$. The reason why we use linear classifier as our model is on two aspects. One is its relatively high efficiency compared with the non-linear model. For a single DCO, its precise distance calculation time complexity is $O(D)$, and the computational efficiency of the model needs to be much smaller than it, while non-linear models usually require complex calculations (exponential, logarithmic operations). The second aspect is its flexibility. We can simply tune parameters such as intercept $\beta$ to ensure that the recall of a certain label reaches the target. Then, we study the effectiveness of linear models and numerical metrics to judge the quality of an approximate distance method.

For a single query $q$ and its $k$ nearest neighbors $u_1,...,u_k$, we set threshold $\tau$ as the distance $\|q,u_k\|$ and we set all visited points during the search process as $S(q)$. With this threshold, the class of Label 0 will be the $u_1,...,u_k$ which is all the $k$ nearest neighbor of $q$ and the class of Label 1 will be $S(q) \setminus u_1,...,u_k$ as the rest of all visited points.
Then we consider the classification recall of a linear model on two classes. It can be seen that the classification recall of class Label 0 directly affects the recall of the $k$ nearest neighbor search algorithm and the recall of class Label 1 affects the efficiency of approximate distance inference. For points classified as Label 0, we still need to calculate their precise distance so that the result queue can maintain the top $k$ results during the search process. For points classified as Label 1, we can avoid precise distance calculations by using approximate distances and the linear model.


For the ANNS search algorithm, a significant reduction in recall is unacceptable. To avoid this situation, we set a recall target of $r$ for Label 0. 
However, the conventional utilization of Binary Cross-Entropy (BCE) loss for training linear models does not guarantee a consistent achievement of a predefined target $\tau$ of recall for label 0. It can be seen that the recall of label 0 is associated with the intercept term $\beta$ of the linear model.

\begin{lem}
    For the linear model $L = sign(m_{1}dis^{\prime} + \beta > \tau)$, as the intercept $\beta$ of the linear model decreases, the recall of label 0 in the training dataset is monotonically non-decreasing.
    \label{lem:increase-recall}
\end{lem}
\begin{proof}
Recall for Label 0 is defined as the ratio of true positives (TP) to the sum of true positives and false negatives (FN). In our case, a true positive is an instance where the model correctly predicts label 0, and a false negative is an instance where the model incorrectly predicts Label 1 when the true Label is 0.
In our linear model $L = sign(m_{1}dis^{\prime} + \beta > \tau)$, a decrease in $\beta$ will shift the decision boundary in a way that more instances are classified as label 0. This means that both the number of true positives and false positives(FP) could potentially increase.

However, since the recall is the ratio of true positives to the sum of true positives and false negatives, an increase in both TP and FP would not decrease the recall, because the ratio would either increase (if the number of true positives increases) or stay the same (if the number of true positives stay the same).
Therefore, we can prove that as the intercept $\beta$ of the linear model decreases, the recall of label 0 in the training dataset is monotonically non-decreasing.
\end{proof}

Since the intercept and recall satisfy the above properties, we can binary search the minimum intercept $\beta$ to satisfy the recall constraint.
Then we consider the efficiency that the linear model can improve by using approximate distance when the classification recall of Label 0 reaches the target $r$.


\subsection{Effectiveness of Linear Model}

\begin{defn}[Pruning Rate]
    Given a query $q$, a linear classifier $L$ and Label 1 dataset $S_1(q)$ in all visited points $S(q)$ during the ANNS process of searching for $q$. The pruning rate $\eta_q$ is defined as:
\begin{equation*}
    \eta_q = \frac{|\{x\in S_1(q)| L(x)=1\}|}{|S_1(q)|}.
\end{equation*}
    i.e., the classification recall of the linear model $L$ for the model with Label 1 in $S(q)$.
\end{defn}

With a certain recall target as a constraint, the average pruning rate $\eta$ of the linear model indicates the effectiveness\footnote{We consider that the exact distance computation for Label 0 ($k$-NN of the query) is unavoidable. Usually, the value of $k$ is small relative to the overall search scale, and this part of the exact distance comparison will not affect the overall efficiency.} of inference using approximate distances. Approximate distance with a higher pruning rate and lower computational cost can achieve DCO operations at a smaller computational cost while having little impact on the search recall of the ANNS algorithm. 

Take the random projection as an example. For a given query $q$ and current point $u$ with a random projection matrix $P$ project into $d$-dimensional space. The approximate distance $dis^\prime = \|P(u), P(q)\|$, and the time complexity is $O(d)$. With a linear model $L_r$ for all visited points $S(q)$ and \textit{pruning rate} $\eta_q$, the total time complexity of fast inference is $O(d \cdot |S(q)| \cdot \eta_q + D \cdot |S(q)| (1-\eta_q))$ where the naive method time complexity is $O(D \cdot |S(q)|)$.

\begin{lem}
    For a given query $q$ and a linear model $L$ with its intercept term $\beta$, as the intercept $\beta$ decreases, the pruning rate $\eta$ of the linear model is monotonic non-increase.
    \label{lem:reduce-eta}
\end{lem}
\begin{proof}
    The definition of pruning rate in our approach can be considered as the ratio between the true negative(TN) and all the negative points (TN+FP). Since Lemma~\ref{lem:increase-recall} proof that a decrease in $\beta$ will cause a monotonic non-decrease in TP and FP. Then the pruning rate (TN)/(FP+TN) will monotonic non-increase.
\end{proof}

Certainly, for approximated distance methods with equivalent computational costs, it becomes evident that a higher pruning rate leads to greater efficiency. Conversely, when the pruning rate remains the same, a lower computational cost is favored. To assess the superior pruning rates among various methods, we adopt a perspective where binary linear models are considered linear reconstructions of approximated distances. Subsequently, we introduce the reconstruction error, defined as follows:

\begin{defn}[Reconstruction Error]
    For a single DCO with $dis^{\prime}$ and $dis$ as the approximate distance and precise distance. With the linear model $L$, the gap between reconstruct distance and precise distance is $\gamma = m \cdot dis^{\prime} + \beta - dis$. Then the reconstruction error is defined as $\epsilon = |m \cdot dis^{\prime} + \beta - dis|^2$.
\end{defn}

It is worth noting that the constraint on recall may equivalently be translated into a constraint on the intercept $\beta$, where $\beta \le \beta_r$. Then the linear model can be considered as a linear transform of the approximate distance $dis^{\prime}$ to $m_1 \cdot dis^{\prime}$. Assume that we have a linear model $L$ such that the reconstruction distance  $\gamma$ follows a zero mean Gaussian distribution, which can be expressed as $\gamma \sim \mathcal{N}(0, \sigma^2)$. From the definition of reconstruction error, the average $\epsilon$ equals $\sigma^2$. we can get the following lemma.

\begin{lem}
    For the linear model $L$ that minimizes the reconstruction error $\epsilon$ with ordinary least squares such that a lower average reconstruction error corresponds to a higher expected pruning rate and higher recall of Label 0 of the linear model.\label{low-error-high-recall}
\end{lem}

\begin{proof} We rewrite the linear model as 
\begin{equation*}
\begin{aligned}
        L(\mathbf{x}) & = sign(m_{1}dis^{\prime} + \beta > \tau) \\
                      & = sign(dis + \gamma > \tau) \\
                      & = sign(\gamma > \tau - dis) \\
\end{aligned}
\end{equation*}
With the assumption that the variables above are independent, the expected pruning rate $\mathbb{E}(\eta)$ is determined by the probability that the equation holds for Label~1 samples as $\mathbb{E}(\eta) = \mathbb{P}(\gamma>\tau-dis)$ where $dis>\tau$ by the definition of Label~1 and pruning rate. The recall expectation of Label~0 is $\mathbb{E}(r)= \mathbb{P}(\gamma \leq \tau-dis)$ where $dis<\tau$. Then we consider the cumulative probability density(CDF) function of the distribution of $\gamma$ as below
\begin{equation*}
F(x) = \frac{1}{2} \left[1 + \text{erf}\left(\frac{x - \mu}{\sigma\sqrt{2}}\right)\right]
\end{equation*}
The $\mathbb{P}(\gamma>\tau-dis)$ can be expressed as $1-F(\tau-dis,\sigma)$ which represents the probability of $\gamma$ distribution in $(\tau-dis, +\infty)$. Similarly, The $\mathbb{P}(\gamma \le \tau-dis)$ can be expressed as $F(\tau-dis,\sigma)$. Now, we need to prove that when average $\epsilon$ is reduced, $F(\tau-dis,\sigma)$ is reduced and the corresponding $1-F(\tau-dis,\sigma)$ is increased.  
Since average $\epsilon$ is equal to $\sigma^2$. Then, we consider the derivative of the error function $\mathrm{erf}$. The definition of the error function is as below
\begin{equation*}
    \mathrm{erf}(x)=\frac2{\sqrt{\pi}}\int_0^x\exp(-t^2)dt
\end{equation*}
The derivative of the error function can be calculated as
\begin{equation*}
    \frac d{dx}\mathrm{erf}(x)=\frac2{\sqrt{\pi}}\frac d{dx}\int_0^x\exp(-t^2)dt=\frac2{\sqrt{\pi}}\mathrm{exp}(-x^2)
\end{equation*}
which is a strictly positive function so the error function is an increase function. Then we can prove this by comparing two gap distributions. Suppose we have two gap distributions $\gamma_0$ and $\gamma_1$ with $\sigma_0$ and $\sigma_1$ which $\sigma_0<\sigma_1$. Consider the Label 1 data which $dis>\tau$ and $\tau - dis<0$. Take the $\tau-dis$ as the $x$ in the CDF function. We have $x<0$ and $\sigma_0<\sigma_1$, then we have 
\begin{equation*}
    \frac{x}{\sigma_0 \sqrt{2}}  < \frac{x}{\sigma_1 \sqrt{2}}
\end{equation*}
Since the error function $\mathrm{erf}$ is an increase function, then we get $F_0(\tau-dis,\sigma_0) < F_1(\tau-dis,\sigma_1)$ and $1-F_0(\tau-dis,\sigma_0) > 1-F_1(\tau-dis,\sigma_1)$ for $dis > \tau$. 
Then we get $\mathbb{P}(\gamma_0 >\tau - dis) > \mathbb{P}(\gamma_1 >\tau - dis)$ and $\mathbb{E}(\eta_0) > \mathbb{E}(\eta_1)$. Similarly, we get $x\ge 0$ with Label 0 data and $F(\tau-dis,\sigma_0) > F(\tau-dis,\sigma_1)$ for $dis \le \tau$. Then we get $\mathbb{P}(\gamma_0 \le \tau-dis) > \mathbb{P}(\gamma_1 \le \tau-dis)$ and $\mathbb{E}(r_0) > \mathbb{E}(r_1)$.
Because average $\epsilon$ equals $\sigma^2$ when average $\epsilon$ reduces the $\sigma^2$ is reduced at the same time. Therefore, we have proved that a linear model $L$ with a lower $\epsilon$ will have a higher expected pruning rate and Label 0 recall.
\end{proof}

It can be noticed that the Label 0 recall may be below the target and we need to shift the $\beta$ to achieve a tradeoff between the pruning rate and recall. Then the mean value of the reconstruction error will not stay zero. To avoid this, we set the intercept change as $\Delta_b$ and convert this change to the threshold, then the expected pruning rate will be $\mathbb{E}(\eta)= \mathbb{P}(\gamma>\tau-dis + \Delta_b)$. As we discuss in Lemma~\ref{low-error-high-recall}, if the $\tau - dis + \Delta_b < 0$ hold for $dis > \tau$ then the relationship between the $\sigma$ and pruning rate still holds. We will study the recall target and the pruning rate with real-world datasets in the analysis section. 

 \begin{figure*}[!t]
	\centering
	\begin{small}
		\subfloat[dim=32]{
            \includegraphics[width=0.48\columnwidth]{./figures/gist_pca_linear_hnsw1_1.png}
            }
		\subfloat[dim=64]{
            \includegraphics[width=0.48\columnwidth]{./figures/gist_pca_linear_hnsw1_2.png}
            }
		\subfloat[dim=128]{
            \includegraphics[width=0.48\columnwidth]{./figures/gist_pca_linear_hnsw1_4.png}
            }
		\subfloat[dim=960]{
            \includegraphics[width=0.48\columnwidth]{./figures/gist_pca_linear_hnsw1_30.png}
            }
		\caption{Example of Linear Model and Distribution}\label{fig:linear_model}
		\vspace{-1mm}
	\end{small}
	\vspace{-1mm}
\end{figure*}

\subsection{Minimize Reconstruction Error}

In the context of utilizing a constrained linear model, when approximating distances with the same computational cost, a lower reconstruction error associated with the approximate distance implies a higher pruning rate. Simultaneously, this signifies that employing the approximate distance with a smaller distance gap variance can yield greater efficiency gains. In the following, we revisit the approach of random projection using a projection matrix. When projecting vectors, our goal is to minimize the error in the projected vectors, aiming for the smallest reconstruction error. In this context, it is essential to select the projection matrix that yields the minimum error among all possible options, akin to the principles of PCA (Principal Component Analysis). Therefore, we employ PCA techniques for approximate distance calculations and the linear model can be viewed as a linear reconstructed approximation of the precise distance. The distributions of sample data are illustrated in Figure~\ref{fig:linear_model}.

It can be observed that with an increase in the projection dimensions, the average reconstruction error decreases, and the approximate distance gradually approaches the precise distance, leading to an increase in the corresponding pruning rate. When the projection dimensions are equal to the original space dimensions (forming a rotated space), samples become linearly separable. The next problem is to determine the optimal projection dimension. To address this, we adopt a strategy similar to Incremental Sampling, employing multiple linear models corresponding to different dimensions.

